Homological Stability for Spaces of Subsurfaces with Tangential Structure

Given a manifold with boundary, one can consider the space of subsurfaces of this manifold meeting the boundary in a prescribed fashion. It is known that these spaces of subsurfaces satisfy homological stability if the manifold has at least dimension five and is simply-connected. We introduce a notion of tangential structure for subsurfaces and give a general criterion for when the space of subsurfaces with tangential structure satisfies homological stability provided that the manifold is simply-connected and has dimension $n\geq 5$. Examples of tangential structures such that the spaces of subsurface with that tangential structure satisfy homological stability are framings or spin structures of their tangent bundle, or $k$-frames of the normal bundle provided that $k\leq n-2$. Furthermore we introduce spaces of pointedly embedded subsurfaces and construct stabilization maps, as well as prove homological stability for these. This is used to prove homological stability for spaces of symplectic subsurfaces.

==> Definition/BoundaryPathswithEnd.tex <==
\begin{defi}
  Let $(e,\mathbf{e})$ denote a thickened boundary path. If we fix a 
  two 
  plane $A$ in $\at{N_M e(I)}{\frac{1}{2}}$, we will denote the 
  restriction 
  of $\mathbf{e}_M$ to $A$ by $\mathbf{e}_A$. We will call a tuple 
  $(e,\mathbf{e}_M,\mathbf{e}_A)$ a \emph{thickened boundary path 
  with a disk}.
  If we furthermore add a tangential structure for the image of 
  $\mathbf{e}_A$ we will call this a \emph{thickened boundary path 
  with a 
  disk with tangential structure}
\end{defi}

==> Example/TangentialStructuresSimplyConnectedFiber.tex <==
\begin{example}
  Examples with simply-connected fiber are given by
\end{example}

==> Lemma/SubsurfaceWithExtraStuffFibration.tex <==
\begin{lemma}
  Suppose $\TopologicalSpace$ is a 
  $\DiffeomorphismGroupBoundary{\Manifold}$-locally retractile space, and 
  $
    Y
    \subset
    \SpaceAllSubsurfaceBoundaryTangential
      {+}
      {\Manifold}
      {\BoundaryConditionTangential{\BoundaryCondition}}
    \times
    \TopologicalSpace
  $
  is a $\DiffeomorphismGroupBoundary{\Manifold}$-invariant subset (where the 
  diffeomorphism group acts from the left on both sides), then
  $\at{\Projection{\TopologicalSpace}}{Y}$ is a locally trivial fibration.
\end{lemma}
\begin{proof}
  
\end{proof}

==> Theorem/HomologicalStabilityParaphrased.tex <==
\begin{theorem}
  
\end{theorem}
